Cavity Light-Matter Entanglement through Quantum Fluctuations

The hybridization between light and matter forms the basis to achieve cavity control over quantum materials. In this work we investigate a cavity coupled to an XXZ quantum chain of interacting spinless fermions by numerically exact solutions and perturbative analytical expansions. We find two important effects: (i) Specific quantum fluctuations of the matter system play a pivotal role in achieving entanglement between light and matter; and (ii) in turn, light-matter entanglement is the key ingredient to modify electronic properties by the cavity. We hypothesize that quantum fluctuations of those matter operators to which the cavity modes couple are a general prerequisite for light-matter entanglement in the groundstate. Implications of our findings for light-matter-entangled phases, cavity-modified phase transitions in correlated systems, and measurement of light-matter entanglement through Kubo response functions are discussed.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> packages.tex <==
\usepackage{float}
\usepackage[usenames,dvipsnames]{color}
%\DeclareGraphicsExtensions{.pdf,.gif,.jpg}
\usepackage[colorlinks=true, citecolor=blue, linkcolor=blue, urlcolor=blue]{hyperref}
\usepackage{bm}
\usepackage{cleveref} %to use \cref command
\usepackage{amsmath,amssymb}
\usepackage{appendix}
\usepackage{lipsum}
\usepackage[usenames,dvipsnames]{color}
%\DeclareGraphicsExtensions{.pdf,.gif,.jpg}
\usepackage{braket}
\usepackage[nottoc,numbib]{tocbibind}
\usepackage{mathtools}
\usepackage{layouts}
\usepackage{lineno}
%\linenumbers

\newcommand{\affiliationRWTH}{
Institut f\"ur Theorie der Statistischen Physik, RWTH Aachen University and JARA-Fundamentals of Future Information Technology, 52056 Aachen, Germany
}
\newcommand{\affiliationMPSD}{
Max Planck Institute for the Structure and Dynamics of Matter,
Center for Free-Electron Laser Science (CFEL),
Luruper Chaussee 149, 22761 Hamburg, Germany
}

\newcommand{\affiliationUNIGE}{
Dipartimento di Fisica, Università di Genova, 16146, Genova, Italy
}
\newcommand{\affiliationCNR}{
SPIN-CNR, 16146, Genova, Italy
}


\usepackage[nolist,nohyperlinks]{acronym}
\begin{acronym}[]
\acro{ll}[LL]{Luttinger liquid}
\acro{cdw}[CDW]{charge-density wave}
\acro{lmc}[LMC]{light-matter coupling}
\acro{td}[TD]{thermodynamic}
\acro{em}[em]{electro-magnetic}
\acro{gs}[GS]{ground-state}
\acro{mf}[MF]{mean-field}
\acro{dmrg}[DMRG]{density matrix renormalization group}
\acro{ed}[ED]{exact diagonalization}
\acro{pt}[PT]{perturbation theory}
\acro{bkt}{Berezinskii–Kosterlitz–Thouless}
\end{acronym}

%\usepackage[subrefformat=parens,labelformat=parens]{subfig}
%Christian
\newcommand{\CE}[1]{\textcolor{green}{{CE: #1 }}}
%Michael
\newcommand{\MS}[1]{\textcolor{cyan}{{MS: #1 }}}
%Giacomo
\newcommand{\GP}[1]{\textcolor{blue}{{GP: #1 }}}
